A communication-avoiding parallel algorithm for the symmetric eigenvalue problem

Many large-scale scientific computations require eigenvalue solvers in a scaling regime where efficiency is limited by data movement. We introduce a parallel algorithm for computing the eigenvalues of a dense symmetric matrix, which performs asymptotically less communication than previously known approaches. We provide analysis in the Bulk Synchronous Parallel (BSP) model with additional consideration for communication between a local memory and cache. Given sufficient memory to store $c$ copies of the symmetric matrix, our algorithm requires $\Theta(\sqrt{c})$ less interprocessor communication than previously known algorithms, for any $c\leq p^{1/3}$ when using $p$ processors. The algorithm first reduces the dense symmetric matrix to a banded matrix with the same eigenvalues. Subsequently, the algorithm employs successive reduction to $O(\log p)$ thinner banded matrices. We employ two new parallel algorithms that achieve lower communication costs for the full-to-band and band-to-band reductions. Both of these algorithms leverage a novel QR factorization algorithm for rectangular matrices.

==> symeig.tex <==

%We study algorithms for computation of the eigenvalue decomposition of a symmetric
%matrix $A=Q^TDQ$ where $Q=(I-YTY^T)$. 
We narrow our consideration to symmetric eigensolver algorithms 
that reduce $A$ to banded form, and rely on known algorithms for reduction from
banded to tridiagonal~\cite{Ballard:2012:CAS:2370036.2145822} and further the computation of the eigenvalues of
the tridiagonal matrix~\cite{Dhillon:2006:DIM:1186785.1186788}. Two-step reduction algorithm (full-to-banded then
banded-to-tridiagonal) have recently been shown to be efficient and practical due
to the lower vertical communication cost associated with the two-step approach~\cite{Auckenthaler2011272}. 
We introduce two new algorithms:
%Our main
%contribution is the introduction of improved techniques for the first step (full-to-banded)
%including
\begin{itemize}
\item a direct full-to-banded reduction approach that performs less interprocessor communication
      but has a higher memory-bandwidth overhead,
\item a parallel successive band reduction approach that can achieve less interprocessor communication
      and less memory-bandwidth than any previously known symmetric eigensolver.
\end{itemize}
%We start with a general formulation of full-to-banded reduction approach that attempts
%to capture the algorithmic space within our consideration. Algorithm~\ref{alg:symeig}
%reduces a full matrix to bandwidth $b$ using a partition function
%$\rho$ where $\rho(A,i)$ yields a sparse matrix $A_i\subset A$ of the same dimensions as $A$ 
%with the sparsity defined by $\rho$. 
%
%\begin{algorithm}
%%\caption{Symmetric Band Reduction}
%\begin{algorithmic}
%\caption {$[Q,B]\gets\text{SE}(A,b,\rho)$}
%\label{alg:symeig}
%\State Require that $A$ is a $n\times n$ dense symmetric matrix and $\rho$ is a matrix partition function
%\State Let $\bar{A}=A$
%\For {$i=1$ to $s$ }
%  \State Compute Householder QR $[Y_i,T_i,R_i]=\rho(\bar{A},i)$
%  \State Compute $W_i=\bar{A}Y_i$
%  \State Compute $U_i=Y_iT_i^T$
%  \State Compute $V_i=\frac{1}{2}U_iW_i^TY_i-W_i$
%  \State Compute $\bar{A} = \bar{A} + U_iV_i^T + V_iU_i^T$
%\EndFor
%\State \textbf{end}
%\State Let $B=\bar{A}$
%\State Let $Q=\prod_{i=1}^s(I-Y_iT_iY_i^T)$
%\State Ensure $A=Q^TBQ$, where $Q$ is orthogonal and $B$ is banded with band width $b$
%\end{algorithmic}
%\end{algorithm}
%
%Specifications of a valid $\rho$ for Algorithm~\ref{alg:symeig} leads to a 
%dependency DAG $G_\text{SE}(\rho)$. Lemma~\ref{lem:seqse} gives the known
%sequential complexity for this algorithm. In the next two sections we build
%up parallel symmetric eigensolve algorithms (subsets of $\rho$) 
%necessary to achieve the communication cost finally given in Theorem~\ref{thm:parse}.

%\begin{lemma}
%\label{lem:seqse}
%Given $n\times n$ dense symmetric matrix $A$, there exists partition $\rho$ such that 
%the sequential cost of $G_{\text{SE}(\rho)}$ is
%$$T(G_{\text{SE}(A,\rho)})=\Theta(\gamma\cdot n^3 + \nu\cdot n^3/\sqrt{H}).$$
%\end{lemma}
%\begin{proof}
%See~\cite{greygeneral2010}.
%\end{proof}




